Equivalence of Dataflow Graphs via Rewrite Rules Using a Graph-to-Sequence Neural Model

In this work we target the problem of provably computing the equivalence between two programs represented as dataflow graphs. To this end, we formalize the problem of equivalence between two programs as finding a set of semantics-preserving rewrite rules from one into the other, such that after the rewrite the two programs are structurally identical, and therefore trivially equivalent. We then develop the first graph-to-sequence neural network system for program equivalence, trained to produce such rewrite sequences from a carefully crafted automatic example generation algorithm. We extensively evaluate our system on a rich multi-type linear algebra expression language, using arbitrary combinations of 100+ graph-rewriting axioms of equivalence. Our system outputs via inference a correct rewrite sequence for 96% of the 10,000 program pairs isolated for testing, using 30-term programs. And in all cases, the validity of the sequence produced and therefore the provable assertion of program equivalence is computable, in negligible time.

==> expresults-lnp.tex <==
\subsection{various stuff}
\FIXME{LNP: some text/comments in a separate file to avoid disrupting your changes. Some ruminations, mostly}.

We use the standard notation $a,\vec a,A$ for scalars, vectors and matrices. Operator type is deduced from the operands.


\paragraph*{Sampling the equivalence space} In our setup, we limit the program size to $x$ nodes, where operators are unary or binary. The total number of programs is $y$ (big number). As we use 500,000 samples for the experiment, we sample $z$ (micro fraction) of the space of vertices only. A more accurate reasoning takes into account the fact that we learn an embedding of the programs along with the pathfinding heuristic. If we consider only the different types of paths of a fixed length, e.g. $l$, we sample $k$ (larger fraction) of the space. These are still small values in regard of the total space size, a key to our success is the regularity and repetitions occuring in this carefully-crafted space.



%% Finding a verifiable program equivalence proof in our framework is now reduced to simply one efficient inference step, in part by accepting to possibly miss some possible equivalences due to the stochastic nature of neural networks.

%% %%% LNP: FIXME: I think I will delete this paragraph, too moonshot.
%% It even shows a first hint of machine intelligence (or machine stupidity), by being able for about 1\% of cases to output an alternate but correct path to the proof than the ``depth-first'' one, a property of paths on which it is being trained. We hope this is a sign the network has learned the generalization of DFS to the more general sequence, but it could be a sign of failure to learn DFS accurately and be correct in these 1\% cases just by luck, too.


==> progequivstatic.tex <==
%% \section{Static Program Equivalence}
%% \label{sec:progequivstatic}
%% \input{progequivstatic}

%%%% LNP ===> FILE DELETED, instead use samplegen.tex.


%% \FIXME{LNP: This section will be totally revisited, to talk only about how to generate equivalent programs w/ steve's (simplified) random algo, and only briefly suggest how one can create a static brute-force checker. Will be done later}

%% Main idea: the brute-force program program equivalence algorithm that enumerates all possible rewrites is the one we make the neural net learn. input/output examples will be used for training, which are random path in the graph this algorithm explore. 


%% It is implicitly learning the algorithm used to generate examples, which is itself an algorithm that can explore the entire set of possible semantics-preserving tree rewrites. In essence, we make the neural network learn the acceleration heuristics to traversing such a space, but by using only classical input/output example-driven training.

%% maybe make a formal def for what is building a random valid path in the graph of transfo to generate program examples, to show it's the same formula for generating programs as it is to prove their equivalence from the previous section defs?


%% \subsection{Enumerating the Space of Equivalent Programs}


%% \subsection{Random Enumeration for Example Generation}

%% \FIXME{LNP: this is where your section currently in 5.1 will go, but I may take/split some parts and put them above. }


%% \subsection{Fast Equivalence Checking with Rewrite Rules}

%% pseudocode for applying the rewrite rule (while ensuring each rw is a valid axiom), and basic dfs-into-list + check lists are equal for the final structural equivalence check


==> related-myold1.tex <==
%% \section{Related Work}
%% \label{sec:related}
%% \input{related}



%% \paragraph*{Program analysis with machine learning}

%% The work presented here is built upon two active research fields: program analysis
%% and generation using machine learning, and graph neural networks for analysis of
%% data which is best represented with graphs. There are recent survey papers
%% summarizing the current state of both of these fields \cite{AllamanisACM18} \cite{Wu19}.

\paragraph*{Theorem provers} The problem of equivalence as we formulated may be solved by other (smart) brute-force approaches, where a problem is solved by pathfinding. This ranges from theoreom proving systems like Coq \cite{bertot2013interactive} which supports the formal framework for equivalence we describe in this paper, to (Approximate Probabilistic) Model Checking \cite{clarke1994model,burch1992symbolic,herault2004approximate}, where a program equivalence system can also be built, e.g. \cite{steffen1991data,clarke2003behavioral,visser2003model,namjoshi2000syntactic}. Our contribution is not in the formal definition of program equivalence we presented, semantics-preserving rewrite systems have been studied, e.g. \cite{visser2004program,lucanu2015program,reddy1989rewriting}. But understanding why this particular formalism was well suited to deep learning graph-to-sequence systems was key.
The merits of stochastic search to accelerate such systems has been demonstrated, e.g. \cite{murawski2005probabilistic,herault2004approximate,gogate2012probabilistic}. The novelty of our approach is to develop carefully crafted graph-to-sequence neural networks to automatically learn an efficient pathfinding heuristic for this problem. Our approach is potentially applicable in these areas too, however training scalability can become a challenge if increasing the input representation size excessively. 

\paragraph*{Static program equivalence} Algorithms for static program equivalence have been developed, e.g. \cite{verdoolaege2012equivalence,alias2004recognition,barthou2002,iooss2014program}. These approaches typically restrict to demonstrating the equivalence of different schedules of the operations, possibly dynamically \cite{bao2016polycheck}. In this work we target graph-modifying rewrites (and therefore which alter the operation count). Barthou et 
al. \cite{barthou2002,alias2004recognition} have developed
techniques to recognize algorithm templates in programs. These
approaches are restricted to static/affine transformed programs.
Karfa et al. also designed a method that works for a subset of affine
programs using array data dependence graphs (ADDGs) to represent input
and transforming behaviors.  Operator-level equivalence checking
provides the capability to normalize expressions and establish
matching relations under algebraic transformations
\cite{karfa2013verification}.  Mansky and Gunter used the TRANS
language \cite{kalvala2009program} to represent transformations.  The
correctness proof implemented in the verification framework
\cite{mansky2010framework} is verified by the Isabelle
\cite{isabelle-web} proof assistant.  Other works
also include translation
validation \cite{sorin:proving,necula2000translation}.


\paragraph*{Program analysis with machine learning} Numerous prior work has employed (deep) machine learning for program analysis, e.g. \cite{AllamanisACM18,Alon19,Tufano19}.
%% PHOG \cite{bielik16} presents a probabilistic
%% grammar to predict node types in an AST.
%
%% While this work does not use machine
%% learning on code, it presents some of the benefits of analyzing code with
%% probability distributions, which is the main strength that machine learning
%% is able to bring to a problem.
code2vec \cite{Alon19} teaches a method for
creating a useful embedding vector that summarizes the semantic
meaning of a snippet of code. Program repair approaches, e.g. \cite{Tufano19,Chen19} are deployed to automatically repair bugs in a program. Output accuracies of up to 20\% on the test set is reported, using sequence-to-sequence models.
Wang et al. \cite{Wang18} learns to extract the rules for Tomita grammars \cite{tomita82} with recurrent neural networks. The learned network weights are processed to create a verifiable deterministic finite automata (DFA) representation of the learned grammar. This work demonstrates that deterministic grammars can be learned with RNNs, which we rely on.
%% , but our network is
%% learning a path finding process which would not easily map onto a DFA.




%% In pe-graph2seq, our rule checker allows us to process the proposed
%% rewrite rule sequences from the neural network. Work by





%% without informing about the semantics rules of programming. 
%% . One of the works \cite{Tufano19}
%% uses a replacement procedure to rename variables to common token for
%% processing by the network; pe-graph2seq presumes a similar process
%% would be used to map arbitrary variable names into the terms
%% used in our grammar. The other work \cite{Chen19} uses an augmentation
%% to the attention mechanism called a copy mechanism \cite{See17}
%% to support rare variable names for the output sequence. Future work
%% on pe-graph2seq could benefit from a copy mechanism as it could
%% allow the system to create equivalence proofs involving variable
%% name changes.


%% Thier technique uses AST analysis, but not
%% graph neural networks.


%% \paragraph*{Program analysis with machine learning}
%% PHOG: Probabilistic model for code \cite{bielik16} presents a probabilistic
%% grammar to predict node types in an AST. While this work does not use machine
%% learning on code, it presents some of the benefits of analyzing code with
%% probability distributions, which is the main strength that machine learning
%% is able to bring to a problem. code2vec \cite{Alon19} teaches a method for
%% creating a useful embedding vector that summarizes the semantic
%% meaning of a snippet of code. Thier technique uses AST analysis, but not
%% graph neural networks.

%% Multiple works have been published on using sequence-to-sequence models
%% to do code repair by generating program fixes as output given a buggy
%% program as input \cite{Tufano19} \cite{Chen19}. These works achieve 
%% output accuracies of up to 20\% on their test set, showing validity
%% to using ML techniques to analyze programs. One of the works \cite{Tufano19}
%% uses a replacement procedure to rename variables to common token for
%% processing by the network; pe-graph2seq presumes a similar process
%% would be used to map arbitrary variable names into the terms
%% used in our grammar. The other work \cite{Chen19} uses an augmentation
%% to the attention mechanism called a copy mechanism \cite{See17}
%% to support rare variable names for the output sequence. Future work
%% on pe-graph2seq could benefit from a copy mechanism as it could
%% allow the system to create equivalence proofs involving variable
%% name changes.

\paragraph*{Graph Neural Networks}
%% The organized nature of computer programs are well represented and analyzed
%% using graphs of various types - abstract syntax trees (ASTs), Control flow
%% graphs (CFGs), etc. \FIXME{Louis-Noel, do you want to cite a paper on that
%% statement?}.
Graph neural networks \cite{Scarselli09,Wu19} use machine learning
to analyze a set of nodes and edges for patterns related to a target problem.
Using a graph-to-sequence network with attention has been analyzed for natural
language processing \cite{Beck18}. Allamanis et al. use graph
neural networks to analyze code sequences and add edge types representing
LastUse, ComputedFrom, and LastWrite to improve the system's ability to
reason about the code \cite{AllamanisICLR18}. Their work achieves 
84\% accuracy on correcting variable misuse cases and provides insights
to useful edge types. %which may be valuable in extending pe-graph2seq to more complex programs.
Structure2vec \cite{Xu17} uses a graph neural network to detect binary code similarity. Structure2vec uses a graph
neural network to learn an embedding from a annotated control flow graph (ACFG)
of a program. This learning process targets the embedding so that equivalent
programs will have equivalent embeddings, reporting precision
scores of 84\% and 85\% on various test datasets for correctly predicting
program equivalence. It only outputs a probability of equivalence, and not a verifiable proof, which is sufficient in their context.
%% which supports our contention
%% that robust program equivalence work with machine learning must involve the
%% creation of an output that creates a proof sequence that confirms 2 programs
%% are equivalent.

%% In our work, each node, including the ProgramCompare node, learns an embedding
%% related to the task of generating a transformation sequence.

The G2SKGE model \cite{Li19} has a similar graph network structure which uses a node embedding (which they refer to as an information fusion mechanism) in order to predict
relationships between nodes. This technique of using a neural network to understand and predict
node interelationships is common to our approach.


==> related-steve.tex <==
%% \section{Related Work}
%% \label{sec:related}
%% \input{related}

The work presented here is built upon two active research fields: program analysis
and generation using machine learning, and graph neural networks for analysis of
data which is best represented with graphs. There are recent survey papers
summarizing the current state of both of these fields \cite{AllamanisACM18} \cite{Wu19}.

\paragraph*{Program analysis with machine learning}
PHOG: Probabilistic model for code \cite{bielik16} presents a probabilistic
grammar to predict node types in an AST. While this work does not use machine
learning on code, it presents some of the benefits of analyzing code with
probability distributions, which is the main strength that machine learning
is able to bring to a problem. code2vec \cite{Alon19} teaches a method for
creating a useful embedding vector that summarizes the semantic
meaning of a snippet of code. Thier technique uses AST analysis, but not
graph neural networks.

Multiple works have been published on using sequence-to-sequence models
to do code repair by generating program fixes as output given a buggy
program as input \cite{Tufano19} \cite{Chen19}. These works achieve 
output accuracies of up to 20\% on their test set, showing validity
to using ML techniques to analyze programs. One of the works \cite{Tufano19}
uses a replacement procedure to rename variables to common token for
processing by the network; pe-graph2seq presumes a similar process
would be used to map arbitrary variable names into the terms
used in our grammar. The other work \cite{Chen19} uses an augmentation
to the attention mechanism called a copy mechanism \cite{See17}
to support rare variable names for the output sequence. Future work
on pe-graph2seq could benefit from a copy mechanism as it could
allow the system to create equivalence proofs involving variable
name changes.

In pe-graph2seq, our rule checker allows us to process the proposed
rewrite rule sequences from the neural network. Work by Wang, \textit{et al.}
\cite{Wang18} learns to extract the rules for Tomita grammars 
\cite{tomita82} with recurrent neural networks. The work then processes
the learned network weights to create a verifiable deterministic finite
automata (DFA) representation of the learned grammar. This work demonstrates
that deterministic grammars can be learned with RNNs, which we rely on,
but our network is learning a path finding process which would not
easily map onto a DFA.

\paragraph*{Graph Neural Networks}
The organized nature of computer programs are well represented and analyzed
using graphs of various types - abstract syntax trees (ASTs), Control flow
graphs (CFGs), etc. \FIXME{Louis-Noel, do you want to cite a paper on that
statement?}. Graph neural networks \cite{Scarselli09} use machine learning
to analyze a set of nodes and edges for patterns related to a target problem.
Using a graph-to-sequence network with attention has been analyzed for natural
language processing \cite{Beck18}. Allamanis, \textit{et al.}, use graph
neural networks to analyze code sequences and add edge types representing
LastUse, ComputedFrom, and LastWrite to improve the system's ability to
reason about the code \cite{AllamanisICLR18}. Their work achieves 
84\% accuracy on correcting variable misuse cases and provides insights
to edge types which may be valuable in extending pe-graph2seq to more complex
programs. The Structure2vec paper \cite{Xu17} uses a graph
neural network to detect binary code similarity. Structure2vec uses a graph
neural network to learn an embedding from a annotated control flow graph (ACFG)
of a program. This learning process targets the embedding so that equivalent
programs will have equivalent embeddings. In their paper they report precision
scores of 84\% and 85\% on various test datasets for correctly predicting
program equivalence, which supports our contention
that robust program equivalence work with machine learning must involve the
creation of an output that creates a proof sequence that confirms 2 programs
are equivalent.

In our work, each node, including the ProgramCompare node, learns an embedding
related to the task of generating a transformation sequence. The G2SKGE model
\cite{Li19}, has a similar graph network structure which uses a node embedding
(which they refer to as an information fusion mechanism) in order to predict
relationships between nodes. While their problem space related to knowledge
graphs, the technique of using a neural network to understand and predict
node interrelationships is common to our approach.

